Data-driven Cloud Clustering via a Rotationally Invariant Autoencoder

Advanced satellite-born remote sensing instruments produce high-resolution multi-spectral data for much of the globe at a daily cadence. These datasets open up the possibility of improved understanding of cloud dynamics and feedback, which remain the biggest source of uncertainty in global climate model projections. As a step towards answering these questions, we describe an automated rotation-invariant cloud clustering (RICC) method that leverages deep learning autoencoder technology to organize cloud imagery within large datasets in an unsupervised fashion, free from assumptions about predefined classes. We describe both the design and implementation of this method and its evaluation, which uses a sequence of testing protocols to determine whether the resulting clusters: (1) are physically reasonable, (i.e., embody scientifically relevant distinctions); (2) capture information on spatial distributions, such as textures; (3) are cohesive and separable in latent space; and (4) are rotationally invariant, (i.e., insensitive to the orientation of an image). Results obtained when these evaluation protocols are applied to RICC outputs suggest that the resultant novel cloud clusters capture meaningful aspects of cloud physics, are appropriately spatially coherent, and are invariant to orientations of input images. Our results support the possibility of using an unsupervised data-driven approach for automated clustering and pattern discovery in cloud imagery.

==> Narrative/00abstract.tex <==
\label{abstract}

\begin{abstract}
Advanced satellite-born remote sensing instruments produce high-resolution multispectral data for much of the globe at a daily cadence.  These datasets open up the possibility of improved understanding of cloud dynamics and feedback, which remain the biggest source of uncertainty in global climate model projections. As a step towards answering these questions, we describe an automated rotation-invariant cloud clustering (RICC) method that leverages deep learning autoencoder technology to organize cloud imagery within large datasets in an unsupervised fashion, free from assumptions about predefined classes. We describe both the design and implementation of this method and its evaluation, which uses a sequence of testing protocols to determine whether the resulting clusters: (1) are physically reasonable, (i.e., embody scientifically relevant distinctions); (2) capture information on spatial distributions, such as textures;  (3) are cohesive and separable in latent space; and (4) are rotationally invariant, (i.e., insensitive to the orientation of an image). Results obtained when these evaluation protocols are applied to RICC outputs suggest that the resultant novel cloud clusters capture meaningful aspects of cloud physics, are appropriately spatially coherent, and are invariant to orientations of input images. Our results support the possibility of using an unsupervised data-driven approach for automated clustering and pattern discovery in cloud imagery.
\end{abstract}

%Advanced satellite-born remote sensing instruments produce high-resolution multi-spectral data for much of the globe at a close to daily cadence.  These datasets open up the possibility of improved understanding of cloud dynamics and feedbacks, which remain the biggest source of uncertainty in global climate model projections. As a step towards answering these questions, we describe an automated rotation invariant cloud classification (RICC) method that leverages deep learning autoencoder technology to identify cloud types within large datasets in an unsupervised fashion, free from assumptions about predefined classes. We describe both the design and implementation of this method and its evaluation, which uses a sequence of testing protocols to determine whether the classes that it identifies:(1) are separable (i.e., are  cohesive in latent space and separated from each other), (2) are stable, i.e., produce similar or identical classes when different subsets of the data are used; (3) capture information on spatial distributions, such as textures; (4) are rotationally invariant, i.e., insensitive to the orientation of an image; and (5) are physically reasonable, i.e., embody scientifically relevant distinctions. Results obtained when these protocols are applied to RICC outputs suggest that the resultant novel cloud classes are appropriately spatially coherent and invariant to orientations of input images, and capture meaningful aspects of cloud physics.

==> Narrative/bios.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Kurihana.jpg}}]{Takuya Kurihana}
(S'21) received the B.S. degree in geoscience from University of Tsukuba, Tsukuba, Japan in 2017, and the M.S. degree in computer science from the University of Chicago, Chicago, United States, in 2020. 
He is currently pursuing the Ph.D. degree in computer science with the University of Chicago, Chicago, United States.

His research interests include remote sensing, machine learning and deep learning with application in remote sensing to climate science. 
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Moyer.jpg}}]{Elisabeth Moyer}
is an associate professor in the Geophysical Sciences department at the University of Chicago. Her research focuses on atmospheric science, climate statistics, and energy and climate policy analysis. Her work includes measurements of high-altitude clouds and climate modeling for impacts assessment, with an emphasis on building statistical tools to help bring climate science results to other fields.
She directs the university's Center for Robust Decision-making on Climate and Energy Policy and the collaborative program ``International Partnership for Cirrus Studies'' and is an associate in the Energy Policy Institute at Chicago.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Becca_IEEE.jpg}}]{Rebecca Willett}
(SM'14) is a Professor of Statistics and Computer Science at the University of Chicago. Her research is focused on machine learning, signal processing, and large-scale data science. 
She is a co-principal investigator and member of the Executive Committee for the Institute for the Foundations of Data Science, helps direct the Air Force Research Lab University Center of Excellence on Machine Learning, and serves on the Scientific Advisory Committee for the National Science Foundation’s Institute for Mathematical and Statistical Innovation and the AI for Science Committee for the US Department of Energy’s Advanced Scientific Computing Research program.
She completed her PhD in Electrical and Computer Engineering at Rice University in 2005 and was an Assistant then tenured Associate Professor of Electrical and Computer Engineering at Duke University from 2005 to 2013. She was an Associate Professor of Electrical and Computer Engineering, Harvey D. Spangler Faculty Scholar, and Fellow of the Wisconsin Institutes for Discovery at the University of Wisconsin-Madison from 2013 to 2018. Willett received the National Science Foundation CAREER Award in 2007, is a member of the DARPA Computer Science Study Group, and received an Air Force Office of Scientific Research Young Investigator Program award in 2010. 
%Willett has also held visiting researcher or faculty positions at the University of Nice in 2015, the Institute for Pure and Applied Mathematics at UCLA in 2004, the University of Wisconsin-Madison 2003-2005, the French National Institute for Research in Computer Science and Control (INRIA) in 2003, and the Applied Science Research and Development Laboratory at GE Healthcare in 2002.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Gilton.jpg}}]{Davis Gilton}
is pursuing a PhD in Electrical and Computer Engineering at the University of Wisconsin-Madison. His research is focused on scalable data science, signal processing, optimization, and deep learning for inverse problems in imaging.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Foster.jpg}}]{Ian Foster}
(F'20) is Senior Scientist and Distinguished Fellow, and director of the Data Science and Learning Division, at Argonne National Laboratory; the Arthur Holly Compton Distinguished Service Professor of Computer Science at the University of Chicago; and a DOE Office of Science Distinguished Scientist Fellow. He has a BSc degree from the University of Canterbury, New Zealand, and a PhD from Imperial College, United Kingdom, both in computer science. His research concerns distributed, parallel, and data-intensive computing technologies, and applications to scientific problems. He is a fellow of the AAAS, ACM, BCS, and IEEE, and has received the BCS Lovelace Medal, the IEEE Babbage, Goode, and Kanai awards, R\&D Magazine's Innovator of the Year award, and honorary doctorates from the University of Canterbury, New Zealand, and CINVESTAV, Mexico.
\end{IEEEbiography}



==> bios.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Kurihana.jpg}}]{Takuya Kurihana}
(S'21) received the B.S. degree in geoscience from University of Tsukuba, Tsukuba, Japan in 2017, and the M.S. degree in computer science from the University of Chicago, Chicago, United States, in 2020. 
He is currently pursuing the Ph.D. degree in computer science with the University of Chicago, Chicago, United States.

His research interests include remote sensing, machine learning and deep learning with application in remote sensing to climate science. 
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Moyer.jpg}}]{Elisabeth Moyer}
is an associate professor in the Geophysical Sciences department at the University of Chicago. Her research focuses on atmospheric science, climate statistics, and energy and climate policy analysis. Her work includes measurements of high-altitude clouds and climate modeling for impacts assessment, with an emphasis on building statistical tools to help bring climate science results to other fields.
She directs the university's Center for Robust Decision-making on Climate and Energy Policy and the collaborative program ``International Partnership for Cirrus Studies'' and is an associate in the Energy Policy Institute at Chicago.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Becca_IEEE.jpg}}]{Rebecca Willett}
(SM'14) is a Professor of Statistics and Computer Science at the University of Chicago. Her research is focused on machine learning, signal processing, and large-scale data science. 
She is a co-principal investigator and member of the Executive Committee for the Institute for the Foundations of Data Science, helps direct the Air Force Research Lab University Center of Excellence on Machine Learning, and serves on the Scientific Advisory Committee for the National Science Foundation’s Institute for Mathematical and Statistical Innovation and the AI for Science Committee for the US Department of Energy’s Advanced Scientific Computing Research program.
She completed her PhD in Electrical and Computer Engineering at Rice University in 2005 and was an Assistant then tenured Associate Professor of Electrical and Computer Engineering at Duke University from 2005 to 2013. She was an Associate Professor of Electrical and Computer Engineering, Harvey D. Spangler Faculty Scholar, and Fellow of the Wisconsin Institutes for Discovery at the University of Wisconsin-Madison from 2013 to 2018. Willett received the National Science Foundation CAREER Award in 2007, is a member of the DARPA Computer Science Study Group, and received an Air Force Office of Scientific Research Young Investigator Program award in 2010. 
%Willett has also held visiting researcher or faculty positions at the University of Nice in 2015, the Institute for Pure and Applied Mathematics at UCLA in 2004, the University of Wisconsin-Madison 2003-2005, the French National Institute for Research in Computer Science and Control (INRIA) in 2003, and the Applied Science Research and Development Laboratory at GE Healthcare in 2002.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Gilton.jpg}}]{Davis Gilton}
is pursuing a PhD in Electrical and Computer Engineering at the University of Wisconsin-Madison. His research is focused on scalable data science, signal processing, optimization, and deep learning for inverse problems in imaging.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Foster.jpg}}]{Ian Foster}
(F'20) is Senior Scientist and Distinguished Fellow, and director of the Data Science and Learning Division, at Argonne National Laboratory; the Arthur Holly Compton Distinguished Service Professor of Computer Science at the University of Chicago; and a DOE Office of Science Distinguished Scientist Fellow. He has a BSc degree from the University of Canterbury, New Zealand, and a PhD from Imperial College, United Kingdom, both in computer science. His research concerns distributed, parallel, and data-intensive computing technologies, and applications to scientific problems. He is a fellow of the AAAS, ACM, BCS, and IEEE, and has received the BCS Lovelace Medal, the IEEE Babbage, Goode, and Kanai awards, R\&D Magazine's Innovator of the Year award, and honorary doctorates from the University of Canterbury, New Zealand, and CINVESTAV, Mexico.
\end{IEEEbiography}


